GORAM: Graph-oriented ORAM for Efficient Ego-centric Queries on Federated Graphs

Ego-centric queries, focusing on a target vertex and its direct neighbors, are essential for various applications. Enabling such queries on graphs owned by mutually distrustful data providers, without breaching privacy, holds promise for more comprehensive results. In this paper, we propose GORAM, a graph-oriented data structure that enables efficient ego-centric queries on federated graphs with strong privacy guarantees. GORAM is built upon secure multi-party computation (MPC) and ensures that no single party can learn any sensitive information about the graph data or the querying keys during the process. However, achieving practical performance with privacy guaranteed presents a challenge. To overcome this, GORAM is designed to partition the federated graph and construct an Oblivious RAM(ORAM)-inspired index atop these partitions. This design enables each ego-centric query to process only a single partition, which can be accessed fast and securely. To evaluate the performance of GORAM, we developed a prototype querying engine on a real-world MPC framework. We conduct a comprehensive evaluation with five commonly used queries on both synthetic and real-world graphs. Our evaluation shows that all benchmark queries can be completed in just 58.1 milliseconds to 35.7 seconds, even on graphs with up to 41.6 million vertices and 1.4 billion edges. To the best of our knowledge, this represents the first instance of processing billion-scale graphs with practical performance on MPC.

==> Makefile <==
PACKAGE=IEEEtran

SAMPLES = \
	main.tex 

PDF = ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.cls %.dtx
	pdflatex -synctex=1 -interaction=nonstopmode $<
	- bibtex $*
	pdflatex -synctex=1 -interaction=nonstopmode $<
	pdflatex -synctex=1 -interaction=nonstopmode $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex -synctex=1 -interaction=nonstopmode $<; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex  
	pdflatex -synctex=1 -interaction=nonstopmode $<
	- bibtex $*
	pdflatex -synctex=1 -interaction=nonstopmode $<
	pdflatex -synctex=1 -interaction=nonstopmode $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex -synctex=1 -interaction=nonstopmode $<; done


# .PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM) *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	*.pdf *.gz *.upa *.upb *.bbl \
	*.pyg

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'



# Makefile for acmart package

# This file is in public domain

# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $


==> intro_ndss.tex <==
\section{Introduction}
\todo{direct present it as queries on fed graphs.}
\todo{outline: 1) problem importance; 2) baseline solutions and their drawbacks (short motivation); 3) our idea.}
A \emph{private federated database} is a system that responds to clients' queries on a collection of databases from mutually distrusting data providers while ensuring that no additional information about each provider is leaked beyond the query result~\cite{bater2017smcql}. 
These databases have emerged as a promising solution that balances data protection and value extraction, thus garnering significant attention from both academia and industry~\cite{liagouris2023secrecy, bater2017smcql, bater2020saqe, volgushev2019conclave}. 

Despite these advancements, current federated databases are primarily designed for conventional tabular data and fall short when it comes to graph data. 
Graphs, with their inherent interconnections, have played an important role in various areas, including financial industry, social networks, public health, \emph{etc}. 
\emph{Ego-centric} queries, \ie queries involving the target vertex and all its direct neighbors, are fundamental in graph applications. 
For instance, commercial banks utilize transaction graphs for efficient detection of money laundering by analyzing relations among suspicious accounts~\cite{neo4financial, qiu2018real}. Social network giants use graphs to model and manage users and their relationships. As LinkBench~\cite{linkbench2013} reports, point reads for accounts, relations, and neighbor-statistics on the given account constitute 12.9\% and 55.6\% of the total processed queries from Meta. In addition, quick identification of people who may have been exposed to an infected person through the contact graph has played an important role during the COVID-19 pandemic~\cite{liu2024making}. 

The above motivating cases reveal that for graph data models, both the graph data and the querying targets contain sensitive information, and we should keep both of them private, necessitating secure computation techniques as prior works on tabular data~\cite{liagouris2023secrecy, bater2017smcql, volgushev2019conclave}.
However, due to the intricate interdependencies among vertices and edges, achieving practical performance presents a unique set of challenges:

% Unlike tabular data, 
In the context of tabular data, we can eliminate unnecessary relations or columns for each SQL query because the \emph{schema} of each data provider is public or at least known to an authorized party~\cite{bater2017smcql, volgushev2019conclave}. 
However, the schema in graph data, which comprises vertices and edges, is an essential part of data to protect~\cite{robinson2015graph}. 
Naively trying to eliminate unnecessary data early unavoidably violates the privacy of data providers.  
Scanning the entire graph for each query is prohibitively expensive, especially for large-scale graphs.

Even though we can reduce the to-be-processed graph sizes for each query, the privacy requirement of the querying keys necessitates a secure indexing mechanism to locate the target sub-graph without revealing the private keys. The existing secure indexing methods, \eg \emph{Oblivious RAM (ORAM)}~\cite{goldreich1996software,zahur2016revisiting}, are designed to access the $i$th element of an array, while keeping the index $i$ secret (Section~\ref{subsec:oram}). 
However, unlike a location-indexed array where each element is independent, the interrelated vertices and edges in a graph make the indexing much more challenging, as we need to extract all the related vertices (or edges) for each query.

Lastly, to achieve real-time responses for large-scale graphs, parallelism is essential, even for plaintext graphs. Secure computation makes the situation even worse, as the secure protocols are inherently slower and involve intensive communication. Enabling parallelisms on graph, however, is more challenging compared to tabular, since we can not simply split the graph into multiple parts and process them independently. 

% what did we do
In this paper, we propose \sysname, a graph-oriented ORAM data structure designed to support efficient ego-centric queries on federated graphs with strong privacy guarantee. 
\sysname is built on top of \emph{secure multi-party computation (MPC)}~\cite{4568207}, a cryptographic technique that allows multiple parties to jointly compute a function on their private inputs, while keeping the inputs secret without a trusted third party. MPC achieves this property by performing secure protocols on the \emph{secret shared} (encoded) data, and the shares are held by non-colluding parties. 
Similar to the prior works on tabular data~\cite{liagouris2023secrecy}, \sysname encodes the graph data and the querying keys as secret shares in the lifecycle of the query process, ensuring that no single party can learn any sensitive information about the query keys or the graph data, including the existing vertices and edges, the number of the neighbors \etc.

To overcome the challenges towards practical performance, the first component of \sysname is a strategic graph partitioning method (Section~\ref{subsec:graph_rep}).  
Specifically, \sysname organizes the graphs into multiple partitions, satisfying that all the information needed for each ego-centric query is contained in \emph{exactly} one partition, and no single party can tell the difference between the partitions. This design enables \sysname to reduce the to-be-processed graph sizes for each query while guaranteeing strong privacy. 
The only information leaked in \sysname is the partition size, which can be padded by the data providers. 
% which only implies the loose upper bounds of the highest vertex degree and the largest \emph{cut-set} size between two vertex groups, see Section~\ref{subsec:security} for details.

At the same time, each partition can be addressed given the vertex ID or edge IDs (\ie source and destination vertices IDs). To enable efficient and secure access to the partitions, \sysname employs an indexing layer on top of the partitions, inspired by ORAM~\cite{zahur2016revisiting} (Section~\ref{subsec:oram-index}). 
Briefly speaking, the indexing layer maintains a secret mapping from the vertex ID or edge IDs to the location of the corresponding partition.
Then, just like the ORAM accessing the $i$th element of an array, \sysname can locate the target partition efficiently without disclosing any information about the querying keys, \ie specific IDs (Section~\ref{subsec:goram-index}). 
 
Besides, \sysname incorporates several optimizations to accelerate both the construction and partition accesses, including a constant-round shuffling protocol and parallelisms. Specifically, \sysname splits the partitions into multiple partition slices, and each slice can be processed in parallel. This design enables parallelism, which is essential for real-time responses on large-scale graphs (Section~\ref{subsec:parall}).

Based on \sysname, we can implement crucial queries easily. 
Through a prototype querying engine built on top of the ABY3~\cite{mohassel2018aby3} MPC framework, we implement five ego-centric queries, including \emph{edge existence}, \emph{1-hop neighbors}, \emph{neighbors statistics} \etc, covering all the queries\footnote{Specifically, query in this paper refers to static query, and we do not support real-time updates yet.} listed in LinkBench~\cite{linkbench2013} (Section~\ref{sec:local_query}).
Then, we evaluate the above queries on five synthetic graphs with varied distributions and three real-world graphs.
Results in Section~\ref{sec:eval} show remarkable efficiency and scalability of \sysname. On synthetic graphs with up to $2^{15}$ vertices, all the basic queries are finished within 132.8 milliseconds, outperforming queries based on prior secure graph data structures by \emph{2 to 3 orders of magnitude}. %\emph{2-to-3-orders-of-magnitude}. 
For a real-world graph, Twitter~\cite{twitter}, with more than 41.6 \emph{million} vertices and 1.4 \emph{billion} edges, the results can be obtained within 35.7 seconds, and the fastest one only takes 58.1 milliseconds. Also, the construction of \sysname only requires 3.0 minutes.
To the best of our knowledge, \sysname is the first step towards querying graphs scaling to more than one \emph{billion} edges in secure computations. 

In summary, our contributions include:

1) We propose \sysname, a graph-oriented ORAM data structure to support efficient sub-linear ego-centric queries on federated graphs guaranteeing strong privacy.

2) We design comprehensive optimizations to enable practical performance on large-scale graphs, including a strategic graph partitioning method, an ORAM-inspired indexing layer, and parallelism support.

3) A prototype querying engine based on \sysname is developed and evaluated comprehensively using five commonly-used queries on eight synthetic and real-world graphs, demonstrating remarkable effectiveness, efficiency, and scalability.

==> protocol/local_proc.tex <==
\begin{algorithm}[t]
	\small
        \SetKwInOut{Config}{\textbf{Global config}}
	\SetKwInOut{Input}{\textbf{Inputs}}
	\SetKwInOut{Output}{\textbf{Output}}
	\caption{\small Local Process }\label{algo:local_process}
        \Config{Vertex set $V$, configuration parameter $k$.}
	\Input{Private graph $G_i = (V_i, E_i), V_i \subseteq V$, for each data provider $P_i$.}
	\Output{2d-partitioned graph $G_i.\sf{Block}$.}
	% \BlankLine
        Computes the vertex chunk number $b = \lceil \frac{|V|}{k} \rceil$\;
        Initiates edge block $G_i.\sf{Block}$ as $b \times b$ empty vectors\;
        \comm{\cfont{Assign edges to the target blocks.}}

        \For{each edge $(v_s, v_d) \in E_i$}{
            Computes the start and end chunk IDs $s=\lceil \frac{v_s}{k} \rceil$ and $e=\lceil \frac{v_d}{k} \rceil$\;
            $G_i.{\sf{Block}}[s][e].{\sf{append}}(v_s, v_d)$ {\cfont{// Attributes can be included.}}\;
        }
        \comm{\cfont{Sort and align each block.}}
        Max block size $l_i \leftarrow max(\{len({\sf{block}}), \forall {\sf{block}} \in G_i.\sf{Block}\})$\;
        \For{each edge $\sf{block}$ $\in G_i.\sf{Block}$}{
            ${\sf{Sort}}({\sf{block}})$ using key $v_s || v_d$\;
            Pads $(l_i - \text{\prot{len}}({\sf{block}}))$ empty edges $(0, 0)$ in the beginning to align with $l_i$\;
        }
        \Return{$G_i.{\sf{Block}}$;}
\end{algorithm}


==> security.tex <==
\input{./table/complexity}


\section{Comparison with Strawman Solutions}\label{sec:analysis}

We analyze the complexity and security of \sysname in Sections~\ref{subsec:eval-complexity} and ~\ref{subsec:security}, respectively. 
For better presentation, we compare \sysname with the two strawman solutions \mat and \elist, based on adjacency matrix and edge list, to demonstrate the superiority of \sysname. 


\subsection{Strawman Solutions}\label{subsec:query-strawman}

\tinypara{Basic queries in \mat. } With the public vertex set $V$, each data provider can locally construct the $|V|^2$ adjacency matrix, encrypt it into the secret shared matrix, and transfer the shares to the computation servers. The computation servers concatenate the secret matrices element-wise to form the whole secret adjacency matrix of $G$, and then build the query engine. 
Similar to \sysname, we model \mat using two ORAMs, \ie \code{VORAM} with $|V|$ rows and \code{EORAM} with $|V|^2$ elements. 
Therefore, for 1) \code{EdgeExist} query on edge $(v_i, v_j)$, we can identify whether it exists by directly extracting the element $(i, j)$ from the \code{EORAM} and comparing it with $0$; 
for 2) \code{NeighborsCount}, we refer to \code{VORAM} and sum up the edge numbers; 
and for 3) \code{NeighborsGet}, we refer to \code{VORAM}, comparing the elements with $0$ through \prot{GT} to eliminate the connectivity strengths, and then directly return to the client. 

\tinypara{Basic queries in \elist. } 
As the vertex IDs are public in our setting, each data provider $P_i$ only has to encrypt their edges $(u, v) \in E_i$ into the secret shared list, with the length of $|E_i| + \epsilon_i$, where $0 \leq \epsilon_i \leq |V|^2 - |E_i|$ is the confusion parameter that can be used to protect the exact edge numbers. We set $\epsilon_i = 0$ to obtain a better performance. 
The computation servers then concatenate each list directly to obtain the $\sum{(|E_i| + \epsilon_i)}$ length whole edge list. Unlike \mat and \sysname, we cannot directly partition the edge list and build the ORAM. Therefore, we scan the \elist for each basic query, the same as the sub-graph process of \sysname while on the whole \elist.


\subsection{Complexity Analysis}\label{subsec:eval-complexity}

Table~\ref{tab:complexity} summarizes the computation and communication rounds complexities using \sysname or the two strawman data structures.
The complexities include three stages: 
1) \emph{Initialization}, which corresponds to the graph integration and data structure construction stages.
2) \emph{Partition access}, note that \elist only has one partition, \ie the whole edge list and 
3) the three \emph{Basic queries} on the partitions, corresponding to Section~\ref{subsec:basic_query}.
We now analyze the superiority of \sysname in terms of complexities.

\tinypara{Comparing with \mat}, \sysname does not rely on the square of vertex set size $|V|^2$, making it suitable for sparse graphs. 
Specifically, the engine construction cost of \mat is $O(N|V|^2)$, due to the $|V|^2$ sized adjacency matrix per provider, limiting scalability for large graphs.
For each online query, \mat requires a sub-graph fetch with at least $O(\log(|V|))$ complexity and up to $O(|V|)$ subgraph processing for \code{NeighborsCount} and \code{NeighborsGet}, restricting performance for sparse graphs, \ie $|E| \ll |V|^2$, which is unfortunately common in the real world, as shown in Figure~\ref{fig:perf_realworld}.
\sysname, however, incurs $O(b^2l\log(l)\log(N))$ engine construction cost while reduces the sub-graph fetches from $O(\log(|V|))$ to $O(\log{b})$ by organizing the graph into 2d-partitions. 
Since $|E| \leq b^2l \ll |V|^2$ for real-world graphs, \sysname achieves superior performance despite sometimes higher query processing complexity (\eg $O(l)$ vs. $O(1)$ for \code{EdgeExist}), as shown in Section~\ref{subsec:eval-performance}.


\tinypara{Comparing with \elist} that traverses the whole edge list $E$ each online query, \sysname reduces the online complexity by reducing the sub-graph sizes through \code{GORAM}, therefore presents much better online processing complexity, especially for dense graphs. By constructing the \code{GORAM} in the offline phase, which incurs higher complexity than \elist since $b^2l \geq |E|$ due to the need for padded empty edges (see Section~\ref{subsec:graph_rep}), \sysname significantly reduces online processing complexities to around $l$ or $bl$ for edge-centric and vertex-centric queries, respectively. Consequently, for each online query, \sysname achieves much better performance, especially for dense graphs, \ie large $|E|$ (Section~\ref{subsec:eval-performance}).

\tinypara{Adaptivity. } As Table~\ref{tab:complexity} shows, the complexities of \mat and \elist are directly related to the vertex numbers $|V|$ or the edge numbers $|E|$, which made them suitable for either excessively dense or sparse graphs. 
However, \sysname offers adaptability by adjusting the configuration parameter $k$ for various distributed graphs, even for the corner cases. Specifically, \sysname adopts to \elist for extremely sparse graphs (\eg \code{1\_regular} graph that each vertex contains at most one edge) by setting $k = |V|$, \ie grouping all the vertices in one group and therefore constructing a $1\times 1$ partition containing the whole edge list; or adopts to \mat for extremely dense graphs (\eg complete graph) by setting $k = 1$. The practical performance superiority keeps aligned with the complexity analysis, shown in Section~\ref{subsec:eval-performance}.


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{./graph/online_performance.pdf}
    \vspace{-.21in}
    \caption{Online Performance Overview}
    \label{fig:online_performance}
\end{figure*}

% \subsection{Security Analysis}\label{subsec:security}

% \para{Security model. } \sysname uses the same security model as ABY3~\cite{mohassel2018aby3}, assuming an \emph{honest majority} and semi-honest adversaries. Specifically, the three computation servers form the \emph{three-party computation (3PC)} servers, which receive the secret shares of the data providers' local data and the querying keys of the client and then carry all the computations through secure protocols. \sysname guarantees that all the proposed protocols are secure in the presence of at most one party corrupted by the semi-honest adversary under the standard simulation-based definitions. 


% \para{Security analysis. } There are two privacy requirements to be satisfied in \sysname, as illustrated in Section~\ref{subsec:principle}. We then show how these two requirements are satisfied.
% For \emph{query key privacy}, it is obvious that the data providers learn nothing about the key. For the computation servers, as they process each basic query through a protocol that is \emph{modular} composed of multiple secure protocols obliviously, \ie independent with the inputs, therefore nothing about the input keys can be learned through its views following \emph{Canetti's composition theorem}~\cite{canetti2000security}.
% \fanxy{I actually want to avoid this privacy definition and analysis, therefore i deleted it in the previous version, as simply, \sysname only reveals the partition size, $l$, all the other information is protected. The following complex yet non-intuitive definition may confuse the readers.}
% For \emph{graph structure privacy}, each data provider $P_i$ locally constructs his graph $G_i$ into a 2d-partitioned secret shared graph, which contains $(\frac{|V|}{k})^2$ edge blocks, and each block contains $l_i$ secret edges. 
% As 3PC guarantees that each secret share $\mathsecret{x}$ is random in the view of the computation servers, the edges in each block are uniformly randomly distributed on $k^2+1$ possible edges (plus one empty edge). 
% Consequently, we can construct a set of random graphs $\mathcal{G}$ by independently sampling each block $l_i$ times from $k^2 + 1$ possible edges. For all graphs $\tilde{G} \in \mathcal{G}$, their secret shares are uniformly random in the view of the computation servers.
% Therefore, the computation servers can not distinguish $G_i$ with any $\tilde{G}$ with advantages from their views. 
% The random set size $|\mathcal{G}| = {(k^2+1)}^{l_i (\frac{|V|}{k})^2}$, and a typical approximation of $|\mathcal{G}| \approx 2^{\Theta({|V|}^2)}$ assuming the edges $|E| \approx \alpha |V|$ for some constant $\alpha$, which is a common assumption for real-world graphs~\cite{chung2010graph}. For details, see Appendix~\ref{app:privacy_sys}.



==> table/security.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[t]
% \small
% \centering
% \caption{Leaked Information of Different Graph Representations}\label{tab:security}
% \vspace{-.1in}
% \resizebox{0.8\linewidth}{!}{
%     \renewcommand{\arraystretch}{1.3}
%     \begin{tabular}{c|ll|ll}
%     \midrule
%     \multirow{2}{*}{Graph Format} &
%       \multicolumn{2}{c|}{Vertices} &
%       \multicolumn{2}{c}{Edges} \\ \cline{2-5} 
%      &
%       \multicolumn{1}{c|}{Leaked info} &
%       \multicolumn{1}{c|}{Servers' view} &
%       \multicolumn{1}{c|}{Leaked info} &
%       \multicolumn{1}{c}{Server's view} \\ \hline \hline
%     \mat &
%       \multicolumn{1}{l|}{Nothing} &
%       $|V_i| = |V|$ &
%       \multicolumn{1}{l|}{Nothing} &
%       \multicolumn{1}{l}{$|E_i| = |E|$} \\ \hline
%     \elist &
%       \multicolumn{1}{l|}{Vertices upper bound} &
%       $|V_i| \leq |E_i|+\epsilon_i$ &
%       \multicolumn{1}{l|}{Edges upper bound} &
%       \multicolumn{1}{l}{$|E_i| \leq |E_i| +\epsilon_i$} \\ \hline
%     \multirow{2}{*}{\sysname} &
%       \multicolumn{1}{l|}{Vertices upper bound} &
%       $|V_i| \leq b*l_i$ &
%       \multicolumn{1}{l|}{Edges upper bound} &
%       \multicolumn{1}{l}{$|E_i| \leq b^2*l_i$} \\ \cline{2-5} 
%      & \multicolumn{1}{l|}{Maximum degree upper bound} & $\max\{\text{deg}(v)\}\leq b*l_i$ & \multicolumn{1}{l|}{\#(same edge) upper bound} & \multicolumn{1}{l}{$\max\{\# e\} \leq l_i$} \\ \hline
%     \end{tabular}
% }
% \end{table*}

